Galaxy Clusters with the Fermi-LAT: Status and Implications for Cosmic Rays and Dark Matter Physics

Galaxy clusters are the most massive systems in the known universe. They host relativistic cosmic ray populations and are thought to be gravitationally bound by large amounts of Dark Matter, which under the right conditions could yield to a detectable $\gamma$-ray flux. Prior to the launch of the Fermi satellite, predictions were optimistic that Galaxy clusters would be established as $\gamma$-ray bright objects by observations through its prime instrument, the Large Area Telescope (LAT). Yet, despite numerous efforts, even a single cluster detection is still pending.

==> Makefile <==
manuscript = ClusterObservationsNagoya

tex_files = $(manuscript).tex

default:
	make clean
	make pdf 
#$(manuscript).dvi

# this mode forces LATEX creation, ignoring errors!
force:
	latex \\nonstopmode\\input $(manuscript)	
	bibtex $(manuscript)
	latex \\nonstopmode\\input $(manuscript)	
	latex \\nonstopmode\\input $(manuscript)	

$(manuscript).dvi: $(tex_files)
	latex $(manuscript)
	bibtex $(manuscript)
	perl compressauthorlist $(manuscript) -n 3
	latex $(manuscript)
	latex $(manuscript)

pdf: 
	pdflatex $(manuscript)
	bibtex $(manuscript)
	perl compressauthorlist $(manuscript) -n 3
	pdflatex $(manuscript)
	pdflatex $(manuscript)
	pdflatex $(manuscript)

#pdf: $(manuscript).dvi
#	dvipdfm -o $(manuscript).pdf $(manuscript)

ps: $(manuscript).dvi
	dvips -o $(manuscript).ps $(manuscript)

ps2pdf: $(manuscript).dvi
	dvips -o $(manuscript).ps $(manuscript)
	ps2pdf $(manuscript).ps $(manuscript).pdf

view: $(manuscript).dvi
	xdvi $(manuscript)

clean:
	rm -f $(manuscript).dvi $(manuscript).aux $(manuscript).bbl \
	$(manuscript).blg $(manuscript).log $(manuscript).ps $(manuscript).pdf

# Check style:
# http://matt.might.net/articles/shell-scripts-for-passive-voice-weasel-words-duplicates/
proof:
	echo "weasel words: "
	sh bin/weasel *.tex
	echo
	echo "passive voice: "
	sh bin/passive *.tex
	echo
	echo "duplicates: "
	perl bin/dups *.tex


==> compressauthorlist <==
#!/usr/bin/perl -w

################################################################################
# Reduces author lists containing more than 8 authors to Bloggs, F., et al., ....
#
# $Id: compressauthorlist,v 1.1 2014/12/12 15:03:27 zimmer Exp $
################################################################################

use strict;
use File::Basename;
use Getopt::Long;
use File::Copy;

my $scriptname = basename($0); # Strip away the leading directory names
my $version = (split / /, q/$Revision: 1.1 $/)[1];

################################################################################
# Handle command line arguments

my $help;
my $man;
my $fieldsperauthor=2;
my $numauthors=8;
Getopt::Long::Configure("bundling");
GetOptions ("help|H"                => \$help,
            "man|M"                 => \$man,
	        "fields-per-author|f=i" => \$fieldsperauthor,
		    "number-of-authors|n=i" => \$numauthors
		       ) or die "$scriptname: Invalid command line option\n";

if ($help || $man || @ARGV != 1) {
    use Pod::Usage;
    if ($man) {
    pod2usage(-verbose => 2);
    }
    else {
    pod2usage(-verbose => 1);
    }
}

################################################################################
# Main part of program

my $infile = $ARGV[0];
$infile = "${infile}.bbl" unless $infile =~ /\.bbl$/;
my $outfile = "/tmp/${scriptname}.bbl";

open INPUT, $infile or die "$scriptname: Cannot open $infile for reading: $!\n";
open OUTPUT, "> $outfile" or die "$scriptname: Cannot open $outfile for writing: $!\n";

my $readingnamelist;
my @namelist;
while (<INPUT>) {
    chomp;
    if (/^{?[A-Z]/) { # Start reading in an author list
    $readingnamelist = 1;
    push @namelist, $_;
    }
    elsif ($readingnamelist) { # Are we already reading an author list?
    if (/^\s*$/) { # When we reach a blank line, stop reading in the author list and process the results
        my $namelist = join " ", @namelist;
	    my $names;
	        my $journal;
		    if ($namelist =~ /^(\D+)(\d\d\d\d.*)$/) { # ApJ style bibliographies
		       $names   = $1;
		       		$journal = $2;
				    }
				        elsif ($namelist =~ /^(.*)(\\emph.*)$/) { # AIP style bibliographies
					      $names   = $1;
					      	       $journal = $2;
						           }
							       my @names = split /,/, $names;
							           if (@names > $fieldsperauthor * $numauthors) {
								      print OUTPUT "$names[$_], " foreach 0..$fieldsperauthor-1;
								      	    print OUTPUT "et al. $journal\n"; # Bloggs, F., et al., .....
									        }
										    else {
										    	 print OUTPUT "$_\n" foreach @namelist; # If there are 8 or fewer authors, just output the data as it was in the original file
											     }
											         print OUTPUT "\n";
												     # Reset variables
												         @namelist = ();
													     $readingnamelist = 0;
													     }
													     else {
													         push @namelist, $_;
														 }
    }
    else {
    print OUTPUT "$_\n";
    }
}

close INPUT;
close OUTPUT;

move($outfile, $infile) or die "$scriptname: Problem moving $outfile to $infile: $!\n";

################################################################################
# Pod documentation

=head1 NAME

compressauthorlist

=head1 SYNOPSIS

compressauthorlist [options] bibliography-file

=head1 DESCRIPTION

This scripts takes a .bbl file (produced by BibTeX), and where a paper has more than a
specified number of authors (default = 8), the author list is reduced to Bloggs, F., et al., ....

=head1 USAGE

Use this script after running B<bibtex> on your manuscript:

 latex manuscript
 bibtex manuscript
 compressauthorlist manuscript
 latex manuscript
 latex manuscript

=head1 OPTIONS

=over 4

=item B<-H, --help>

Display a brief help message

=item B<-M, --man>

Display more detailed help

=item B<-f, --fields-per-author=VALUE>

The number of fields in the comma-separated list of names in the .bbl that correspond to
a single author (default = 2: Bloggs, F., Soap, J., ...)

=item B<-n, --number-of-authors=VALUE>

Number of authors above which the author list is to be compressed (default = 8)

=back

=head1 VERSION

This is compressauthorlist $Revision: 1.1 $

=head1 AUTHOR

David Henley <dbh@physast.uga.edu>

=cut



################################################################################
# $Log: compressauthorlist,v $
# Revision 1.1  2014/12/12 15:03:27  zimmer
# First skeleton draft with cartoon figures.
#
# Revision 1.7  2008/10/07 16:05:38  dbh
# Now works if there are {}'s around the authors' names.
#
# Revision 1.6  2008/10/06 14:32:58  dbh
# Added to documentation.
#
# Revision 1.5  2008/08/14 21:54:59  dbh
# Minor correction to documentation.
#
# Revision 1.4  2008/07/18 13:10:26  dbh
# Added --fields-per-author option and ability to deal with AIP-style
# bibliographies.
#
# Revision 1.3  2007/07/19 23:03:30  dbh
# Made sure all dies had $scriptname and \n in them.
#
# Revision 1.2  2007/03/01 22:36:36  dbh
# Added -n (--number-of-authors) option.
#
# Revision 1.1  2007/02/15 16:50:27  dbh
# Initial revision
#

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

